SRG/eROSITA Survey in the Lockman Hole: Classification of X-ray Sources

We have classified the point-like X-ray sources detected by the SRG/eROSITA telescope in the deep Lockman Hole survey. The goal was to separate the sources into Galactic and extragalactic objects. In this work have used the results of our previous cross-match of X-ray sources with optical catalogs. To classify SRG/eROSITA sources we have used the flux ratio $F_{x}/F_{o}$ and information about the source optical extent. As a result, of the 6885 X-ray sources in the eROSITA catalog 357 sources have been classified as Galactic and 5929 and as extragalactic. 539 out of 6885 have been treated as hostless, i.e., having no optical counterparts in the optical catalogs under consideration. 60 have remained unclassified due to the insufficient reliability of optical photometry. Recall and precision for the extragalactic sources are 99.9 and 98.9% (respectively) and 91.6 and 99.7% for the Galactic sources. Using this classification, we have constructed the curves of cumulative number counts for the Galactic and extragalactic sources in the Lockman Hole field. The code that accompanies this paper is available at https://github.com/mbelveder/ero-lh-class.git.

==> figures/nnmag_table.tex <==
\begin{tabular}{c|cccc}
Model         & Features                                                                                & Sample size$^1$                                               & Network structure                                                                    & Overall quality$^2$ \\\hline\hline
nnmag\_grzw1w2 & \begin{tabular}[c]{@{}c@{}}g,r,z, w1, w2\\ g-r,r-z,g-z\\ z-w1, r-w1, w1-w2\end{tabular} & \begin{tabular}[c]{@{}c@{}}1: 10480\\ 0: 55636\end{tabular}  & \begin{tabular}[c]{@{}c@{}}4 layers with 8 neurons\\ Dropout rate: 0.1\end{tabular}  & 0.67           \\\hline
nnmag\_grzw1   & \begin{tabular}[c]{@{}c@{}}g,r,z, w1\\ g-r,r-z,g-z, z-w1\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}1: 10814\\ 0: 89670\end{tabular}  & \begin{tabular}[c]{@{}c@{}}4 layers with 8 neurons\\ Dropout rate: 0.1\end{tabular}  & 0.61           \\\hline
nnmag\_grz     & \begin{tabular}[c]{@{}c@{}}g,r,z\\ g-r,r-z,g-z\end{tabular}                             & \begin{tabular}[c]{@{}c@{}}1: 11092\\ 0: 141845\end{tabular} & \begin{tabular}[c]{@{}c@{}}2 layers with 13 neurons\\ Dropout rate: 0.0\end{tabular} & 0.38      
\end{tabular}

==> figures/quality_table.tex <==

\begin{tabular}{c|cccccc}
Model                                                                                          & \begin{tabular}[c]{@{}c@{}}Companion\\ is correct\\ (A)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Companion\\ is incorrect\\ (B)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Companion \\ assigned\\ to hostless\\ (C)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Source \\ with companion\\ assigned hostless\\ (D)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Correct\\ hostless\\ (E)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ quality\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}NWAY + \\ nnmag\\ $p_{\rm any, 0} = 0.12$\end{tabular}                   & 503                                                              & 20                                                                 & 6                                                                                    & 6                                                                                               & 24                                                              & Q = 0.94                                                   \\ \hline
\begin{tabular}[c]{@{}c@{}}closest\\ candidate\\ $p_{\rm any, 0} = 0.24$\end{tabular}               & 460                                                              & 61                                                                 & 9                                                                                   & 8                                                                                               & 21                                                              & Q = 0.86                                                   \\ \hline
\begin{tabular}[c]{@{}c@{}}NWAY + \\ nnmag\\ (bright sources)\\ $p_{\rm any, 0} = 0.11$\end{tabular} & 246                                                              & 4                                                                  & 0                                                                                    & 0                                                                                               & 3                                                               & Q = 0.98                                                   \\ \hline
\end{tabular}


==> tables/qso_outliers.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{llrrlllrrrlrr}
\toprule
{} &            srcname\_fin &      DL & p\_any & SDSS\_class & MILQ\_class &                OTYPE\_V & SDSS\_z & MILQ\_z & SIMBAD\_z & MILQ\_ZCITE & lg(Fx/Fo) &  color \\
\midrule
\hline
0 &  SRGe J104043.9+593414 &  17.724 & 0.979 &         -  &        QSO &       Seyfert 2 Galaxy &     -  &  0.148 &       -  &     0887   & 1.677 & -2.038 \\
1 &  SRGe J102535.1+570807 &  11.163 & 0.912 &         -  &        QSO &                 Galaxy &     -  &  0.027 &    0.027 &     2MAGN  & 0.490 & -3.029 \\
2 &  SRGe J103408.7+600148 & 153.821 & 0.970 &        QSO &        QSO &       Seyfert 2 Galaxy &  0.051 &  0.051 &    0.051 &     DR14   & 0.398 & -1.886 \\
3 &  SRGe J104949.3+593437 &  21.435 & 0.982 &        QSO &        QSO &                 Quasar &  3.539 &  3.539 &    3.539 &     DR16Q  & 0.182 & -1.438 \\
4 &  SRGe J105348.7+570659 &  20.362 & 0.020 &         -  &        QSO &  Active Galaxy Nucleus &     -  &  0.006 &       -  &     DR16   & 0.151 & -3.064 \\
\bottomrule
\end{tabular}}

==> tables/tp_fp.tex <==
\begin{tabular}{c|lcc}
\multicolumn{2}{c}{\multirow{2}{*}{}}             & \multicolumn{2}{c}{Предсказанный класс}   \\
\cline{3-4}
\multicolumn{2}{c}{}                              & внегалакт. & \multicolumn{1}{l}{галакт.} \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{\makecell{Реальный\\ класс}}} & \multicolumn{1}{c}{внегалакт.} & 2529  & 1                       \\
                      & галакт.                       & 28    & 306                    
\end{tabular}

==> tables/z_stars.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{llrllllrrrl}
\toprule
{} &            srcname\_fin &     p\_any & GAIA\_class & SDSS\_class & MILQ\_class &                  OTYPE\_V &   SDSS\_z & MILQ\_z &  SIMBAD\_z &                 SDSS\_NAME \\
\hline
\midrule
0 &  SRGe J104605.8+583909 &  0.871524 &       STAR &       STAR &       STAR &  Double or Multiple Star &  0.00027 &     -  &        -  &  SDSS J104606.35+583907.8 \\
1 &  SRGe J105327.0+583221 &  0.635770 &       STAR &       STAR &         -  &            Low-mass Star & -0.00010 &     -  &        -  &  SDSS J105327.36+583220.1 \\
2 &  SRGe J103410.4+580344 &  0.018406 &       STAR &     GALAXY &     GALAXY &         Starburst Galaxy &  0.00747 &  0.007 &        -  &  SDSS J103410.15+580349.1 \\
3 &  SRGe J103224.9+572814 &  0.970368 &       STAR &        QSO &        QSO &                   Quasar &  2.43363 &  2.428 &  2.433591 &  SDSS J103224.99+572814.1 \\
4 &  SRGe J105848.1+592918 &  0.887850 &       STAR &         -  &         -  &               HII Region &       -  &     -  &  0.022110 &                        -  \\
\bottomrule
\end{tabular}
}
